Detection of substructure with adaptive optics integral field spectroscopy of the gravitational lens B1422+231

Strong gravitational lenses can be used to detect low mass subhalos, based on deviations in image fluxes and positions from what can be achieved with a smooth mass distribution. So far, this method has been limited by the small number of (radio-loud, microlensing free) systems which can be analysed for the presence of substructure. Using the gravitational lens B1422+231, we demonstrate that adaptive optics integral field spectroscopy can also be used to detect dark substructures. We analyse data obtained with OSIRIS on the Keck I Telescope, using a Bayesian method that accounts for uncertainties relating to the point spread function and image positions in the separate exposures. The narrow-line [OIII] fluxes measured for the lensed images are consistent with those measured in the radio, and show a significant deviation from what would be expected in a smooth mass distribution, consistent with the presence of a perturbing low mass halo. Detailed lens modelling shows that image fluxes and positions are fit significantly better when the lens is modelled as a system containing a single perturbing subhalo in addition to the main halo, rather than by the main halo on its own, indicating the significant detection of substructure.The inferred mass of the subhalo depends on the subhalo mass density profile: the 68% confidence interval for the perturber mass within 600 pc are: 8.2$^{+0.6}_{-0.8}$, 8.2$^{+0.6}_{-1}$ and 7.6$\pm0.3$ $\log_{10}$[M$_{\rm{sub}}$/M$_\odot$] respectively for a singular isothermal sphere, a pseudo-Jaffe, and an NFW mass profile. This method can extend the study of flux ratio anomalies to virtually all quadruply imaged quasars, and therefore offers great potential to improve the determination of the subhalo mass function in the near future.

==> Makefile <==
paper: ms.pdf

clean:
	-rm -f *.aux *.log *.dvi *.bbl *.blg *.tex~ *.ps 

all: goods_sub_mags.pdf plan.pdf,goods_sub_outline2.pdf ms.pdf checkFigures.pdf

allps: goods_sub_mags.ps plan.ps goods_sub_outline2.ps ms.ps checkFigures.ps


# ----------------------------------------------------------------------------

# Postscript output from latex - figures need to be eps!
goods_sub_mags.dvi: goods_sub_mags.tex macros.tex references.bib
	latex goods_sub_mags.tex
	latex goods_sub_mags.tex
	bibtex goods_sub_mags
	latex goods_sub_mags.tex
	latex goods_sub_mags.tex
goods_sub_mags.ps: goods_sub_mags.dvi 
	\dvips -t letter -o goods_sub_mags.ps goods_sub_mags.dvi

goods_sub_mags.pdf: goods_sub_mags.dvi
	\dvipdf -sPAPERSIZE=letter goods_sub_mags.dvi
##################################################################



#ms3.dvi: ms3.tex macros.tex references.bib
#	latex ms3.tex
#	latex ms3.tex
#	bibtex ms3
#	latex ms3.tex
#	latex ms3.tex
#ms3.ps: ms3.dvi 
#	\dvips -t letter -o ms3.ps ms3.dvi

#ms3.pdf: ms3.dvi
#	\dvipdf -sPAPERSIZE=letter ms3.dvi


ms3.bbl: ms3.tex macros.tex references.bib
	./bubble.txt -f ms3.tex references.bib >& ms3.bbl.log
	cat ms3.bbl.log

ms3.dvi: ms3.bbl ms3.tex macros.tex
	#pdflatex ms3.tex
	#pdflatex ms3.tex	
	latex ms3.tex
	latex ms3.tex
	
ms3.ps: ms3.dvi 
	\dvips -t letter -o ms3.ps ms3.dvi

ms3.pdf: ms3.dvi
	\dvipdf -sPAPERSIZE=letter ms3.dvi
	
	
	
	






############
plan.dvi:plan.tex 
	latex plan.tex
	
plan.ps:plan.dvi 
	\dvips -t letter -o plan.ps plan.dvi
#######

checkFigures.dvi: checkFigures.tex macros.tex references.bib
	latex checkFigures.tex
	
checkFigures.ps: checkFigures.dvi 
	\dvips -t letter -o checkFigures.ps checkFigures.dvi

checkFigures.pdf: checkFigures.dvi
	\dvipdf -sPAPERSIZE=letter checkFigures.dvi







==> macros.tex <==
\def\apj{ApJ}
\def\mnras{MNRAS}
\def\apjl{ApJL}
\def\apjs{ApJS}
\def\araa{ARAA}
\def\aap{A\&A}
          

\def\paperone{N11}
\def\GC{GOODS/COSMOS}


\def\galfit{{\sc galfit }}
\def\hst{{\it HST }}
\def\sextractor{{\sc SExtractor }}


\def\eg{{\it e.g.\ }}
\def\ie{{\it i.e.\ }}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\zband{$z_{850}$-band }
\def\vband{$v_{606}$-band }
\def\z8{$z_{850}$}
\def\z{z$_{850}$}
\def\I{I$_{814}$}
%\def\i{i$_{775}$}
\def\isub{i$^{+}$}

\newcommand{\bs}{\boldsymbol}
\newcommand{\mc}{\mathcal}
\newcommand{\true}[1]{\widehat{#1}}

\def\TODO#1#2{{\bf TODO: {#1}: {#2}}}
\def\QUERY#1#2{{\bf QUESTION: {#1}: {#2}}}

\def\sun{\odot}
\def\Msun{M_\odot}
\def\ss{SML}
\def\ls{LS}
\def\Mstar{M^{*}}
\def\rtwo{R_{200}}


%%% general modelling things
\def\modpars{\bs{\theta},\bs{\Lambda}}
\def\allDat{\bs{D}}
\def\data{\bs{d}}


%parameters for the spatial distribution
\def\spatpars{\bs{\theta}}
\def\epss{\epsilon_{\rm s}}
\def\rpower{\gamma_{\rm p}}
\def\qfrac{f_{\rm q}}
\def\pars{\bs{\theta}_{\rm s}}
\def\phispiral{\phi_{\rm sp}}
\def\phiel{\phi_{\rm el}}
\def\dtheta{\phi}
\def\pos{\bs{x}}
\def\Rsat{R_{\rm sat}}
\def\Rmin{R_{\rm min}}
\def\Rmax{R_{\rm max}}



%%%Satellite Luminosity Fn:
% Schechter function parameters:
\def\alphas{\alpha_{\rm s}}
\def\Lsat{L_{\rm s}}
\def\lamo{\lambda_{\rm o}}
\def\lam{\lambda}
\def\mi{I_{814}} 
\def\mz{z_{850}} 
\def\mmax{m_{\rm{max}, j}}
\def\nobs{N^{\rm obs}}
\def\mumax{\mu_{\rm max}}
\def\mumin{\mu_{\rm min}}
\def\nobjs{N}
\def\dm{\Delta m}

%Satellite Number Parameters:
\def\numsat{N_{\rm{s} }}

%Background Properties:
\def\parb{\bs{\theta}_b}
\def\densb{\Sigma_b}
\def\sigdensb{\sigma_{b,cos}}
\def\alphab{\alpha_{\rm b}}
\def\numbak{N_{\rm b}}
\def\numbakobs{N_{\rm b,obs}}
\def\numbakmod{N_{rm b, mod}}


\def\cosvar{\xi}
\def\cosvarnorm{\xi_{\rm o}}
\def\cosvarpower{\delta}
\def\mmax{m_{\rm max}}

% Host galaxy properties:
\def\epsh{\epsilon_{\rm h}}
\def\hdat{\bs{h}}
\def\numhosts{N_{\rm h}}
\def\Lhost{L_{\rm h}}
\def\Rhost{R_{\rm h}}
\def\Rh{$R_{\rm h}$}
\def\Rvir{R_{200}}
\def\Mvhost{M_{\rm v, h}}
\def\MstarHost{M^{*}_{\rm h}}
\def\Mvir{M_{vir}}


%probability:
\def\sat{S}
\def\back{B}
\def\prob{{\rm Pr}}
\def\Gauss{{\rm G}}

%completeness
\def\nobjscorrect{\hat{N}_{\rm c}}


